Block-Value Symmetries in Probabilistic Graphical Models

One popular way for lifted inference in probabilistic graphical models is to first merge symmetric states into a single cluster (orbit) and then use these for downstream inference, via variations of orbital MCMC [Niepert, 2012]. These orbits are represented compactly using permutations over variables, and variable-value (VV) pairs, but they can miss several state symmetries in a domain. We define the notion of permutations over block-value (BV) pairs, where a block is a set of variables. BV strictly generalizes VV symmetries, and can compute many more symmetries for increasing block sizes. To operationalize use of BV permutations in lifted inference, we describe 1) an algorithm to compute BV permutations given a block partition of the variables, 2) BV-MCMC, an extension of orbital MCMC that can sample from BV orbits, and 3) a heuristic to suggest good block partitions. Our experiments show that BV-MCMC can mix much faster compared to vanilla MCMC and orbital MCMC.

==> compute.tex <==
\section{COMPUTING BV SYMMETRIES}


We now discuss how to compute Block-Value symmetries for a given graphical model. Following previous work for computation of Variable and VV Symmetries, the computation of BV-Symmetries is reduced to finding the automorphic group of an appropriately defined coloured graph. For now we assume a specific block partition as input. We discuss heuristics for computing good partitions in Section \ref{}. 

Given a graphical model $\G=\{(f_j,w_j)\}_j$ and a block partition $\Delta=\{B_1,B_2..B_m\}$, the colored graph $G_{BV}^{\Delta}$ is defined by adding a hub node for each block $B_i \in \Delta$. One node each is also added for every assignment $b_i^k \in \mathcal{V}(B_i)$ of every block $B_i$. As before in VV Symmetries, a node is also added for each formula $f_j$. When assigning colours,  all hub nodes are assigned the same colour. Similarly, all nodes representing values of a block are also assigned the same colour similar to value nodes in '
	VV Symmetries. Each formula node $f_j$ is assigned a colour based on weight $w_j$, where each weight is assigned a unique colour. Adding edges, all hub nodes for each block $B_i$ are connected to their respective value nodes. A value node $b_i^k$ of a Block $B_i$ is connected to a formula node $f_j$ if that block's parti	al assignment makes the formula $f_j$ true. Figure \ref{} shows a colored graph for the graphical model ?.

Any graph isomorphism software (like Saucy \cite{saucy}) can be run over the coloured graph $G_{BV}^{\Delta}$ to get the generators for the  automorphism group of this graph. We use this automorphism group directly to get the automorphism group of BV for the symmetries graphical model $\G$ under a block partition $\Delta$.

\begin{thm}
Any permutation $\psi$ that preserves graph automorphism in coloured graph $G_{BV}^{\Delta}$ is a BV symmetry of $\G$ for block partition $\Delta$
\end{thm}

\begin{thm}
The automorphic group of colored graph $G_{BV}^{\Delta}$ is a BV automorphic group $\Psi_{\G}^{\Delta}$ of graphical model $\G$ for block partition $\Delta$
\end{thm}


\begin{comment}
\begin{algorithm}
\caption{Algorithm for generating auxilliary graph for automorphism}\label{get_aux_graph}
\begin{algorithmic}[1]
\Procedure{Get-Aux-Graph}{ 
\newline $\mathcal{G}$=$\{f_j,w_j\}$ \Comment{Graphical model $\mathcal{G}$}
\newline $\Delta$=$\{B_1,B_2..B_m\}$ \Comment{Block Partition $\Delta$}
\newline}
\State Initialise a graph $\G_{aux}$
\For{$\{f_j,w_j\} \in \G$}
\State Add a node $\{f_j\}$ to $\G_{aux}$ with colour $w_j$. 
\EndFor
\For{$B_i$ $\in$ $\Delta$}
\State Add a node $Hub_i$ to $\G_{aux}$.
\For{$b_i^j \in \mathcal{V}_i$}
	\State Add a node ($B_i$, $b_i^j$) to $\G_{aux}$ with colour ($\mathcal{V}_i$)
\For{$f_j \in \G$}
	\State Add an edge between $\{f_j\}$ and $b_i^j$ if the partial assignment ($B_i$, $b_i^j$) makes $f_j$ true.
\EndFor

\EndFor
\EndFor
\State \Return{$\mathcal{G}_{aux}$}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{comment}
